LakeFM: Toward a Foundation Model for Aquatic Ecosystems Using Irregular Multivariate Multi-depth Time Series Data

Understanding and forecasting lake dynamics is critical for monitoring water quality and ecosystem health across lakes and reservoirs. While machine learning methods have been recently applied to ecological time-series data, existing works assume regular sampling in time and depth, and struggle to generalize across lakes with heterogeneous variables, depths, and observation patterns. To address these limitations, we introduce \textsc{LakeFM}, a foundation model for aquatic systems, pre-trained on large-scale ecological datasets comprising both simulated and observed lakes. Through extensive empirical evaluation, we show that \textsc{LakeFM} learns meaningful representations spanning broader lake-level characteristics, and achieves competitive or often superior-forecasting performance compared to existing time-series foundation and non-foundation models, while producing physically plausible predictions consistent with real-world lake dynamics.

==> questions.tex <==
\section{Questions}

\begin{enumerate}
    \item \question{In Figure~\ref{fig:lake_summary}, we consider the geographical region feature to look for lake embedding clustering. Is geographic clustering meaningful and informative? Are there other features that we can consider for clustering?}
    
    \item \question{In Table~\ref{tab:ablation_inputs_compact} (BARC), removing either DO or temperature results in identical MSE when predicting DO. Does this suggest a strong correlation or redundancy between temperature and DO? Is this reasonable?}

    \item \question{In Figure~\ref{fig:per_lake_delta_heatmaps}, for Lake BARC we observe that removing DO as an input improves prediction performance for both DO and temperature. Is this behavior expected? If yes, what characteristics could explain this effect?}

    \item \question{In Figure~\ref{fig:per_lake_delta_heatmaps}, for Lake GL4 we observe that masking any input variable leads to improved prediction performance for PAR. Is it a characteristic of PAR or there is something specific about GL4?}

    \item \question{In Figure~\ref{fig:per_lake_delta_heatmaps}, for Lake TB,  masking any input variable degrades the prediction performance for chlorophyll-a, whereas masking chlorophyll-a has little effect on the prediction of other variables. How can this behavior be interpreted? Except for maybe, BM and CB, Chla is affected negatively by the masking of any variable. Can we say that Chla is a highly dependent variable out of all/or the most sensitive ?}

    \item \question{From Figure \ref{fig:per_lake_delta_heatmaps_v1}, especially BVR and CB, can we say that chlorophyll is a highly dependent variable (similar to the previous observation) and is very sensitive to the addition of other variables? Is this expected/observed generally in literature?}
    
    \item \question{In ~\ref{fig:per_lake_delta_heatmaps} several lakes (WI, Sugg, GL4, FCR (small improvement), CB, BVR, and BARC), masking DO improves temperature prediction performance. Is there any reason?}

    \item \question{In Figure~\ref{fig:prla_masking}, masking temperature at deeper depths leads to a larger degradation in prediction performance compared to shallow depth (3m vs. 1m). Additionally, temperature masking reduces predictive uncertainty (narrower confidence intervals).}

    \item \question{Shallow or Deeper (Figure \ref{fig:cram_masking_deeper_viz}, \ref{fig:cram_masking_shallow_viz}, \ref{fig:barc_depth_masking_viz}) Depth masking doesn't seem to affect the variates that much. In general, is it possible to recover the variables based on whatever depths available? i.e. do they have a good correlation across depths such that a model can infer the predictions even with variables at certain depths missing?}

    \item \question{Figure \ref{fig:lake_pairs_1} - In 2022, BM and CB are similar throughout except during the summer. This is also visible in 2021 (d) and 2020 (e), although in 2019, the deviation starts late summer. CR and BM, on the other hand, are similar throughout (Figure \ref{fig:lake_pairs_2} (i, j, k). We also see, CR and CB are similar (l, m). So, my question is, if CR is similar to both CB and BM, can I not expect CB and BM to be similar as well ? The dissimilarity is arising mainly during the summer months. Is there any known reason for this?}

    \item \question{In Figure \ref{fig:lake_pairs_3}, SP and CB are similar in 2021, but different for 2018, 2019, 2022. Is there any reason for this? }

    \item \question{Are there any observations/interpretations that we can draw from Figures \ref{fig:trajectories_2020_2022}, \ref{fig:trajectories_2018_2020}, \ref{fig:trajectories_2014_2017}?}

    \item \question{In Figure \ref{fig:variable_masking}, we plot the trajectory considering just 1 input variable. What kind of observations can we draw or what should we be looking in such plots? Are we looking into the trajectory similarities to figure out the dominant variables?}
\end{enumerate}


